Resolution studies with the DATURA beam telescope

Detailed studies of the resolution of a EUDET-type beam telescope are carried out using the DATURA beam telescope as an example. The EUDET-type beam telescopes make use of CMOS MIMOSA 26 pixel detectors for particle tracking allowing for precise characterisation of particle sensing devices. A profound understanding of the performance of the beam telescope as a whole is obtained by a detailed characterisation of the sensors themselves. The differential intrinsic resolution as measured in a MIMOSA 26 sensor is extracted using an iterative pull method and various quantities that depend on the size of the cluster are discussed: the residual distribution, the intra-pixel residual-width distribution and the intra-pixel density distribution of track incident positions.

==> content/beam_lines.tex <==

For this work, data have been taken at the \mbox{DESY-II} test beam facilities. 
% Test beam in general and at DESY
%Test beam facilities have shown up as working horses for detector development for LHC upgrades as well as the future linear colliders.
The \mbox{DESY-II} electron/positron synchrotron at the DESY site in Hamburg has a circumference of 292.8\,m and is mainly used as an injector for the PETRA-III storage ring. 
However, it also supplies beam to three test beam areas, one  of them being the test beam area~21.
Its dipole magnets operate in a sinusoidal ramping mode with a frequency of 12.5\,Hz. 
Therefore, one \mbox{DESY-II} cycle takes 80\,ms, and the bunch length is around 30\,ps. 
% Principle of Test beam generation 
The \mbox{DESY-II} synchrotron is equipped with movable carbon fibres. 
If positioned in the beam, bremsstrahlung photons are created, escaping the beam line tangentially.
Subsequently, the photons are converted to electron/positron pairs on a secondary metal target. 
Their energy distribution reaches up to 6\,GeV. 
Using a dipole magnet, this secondary electron/positron beam is spread out.
A collimator can be used to select certain energy ranges of the beams reaching the experimental halls with an achievable rate of about $10$\,kHz to $100$\,kHz. 
A more detailed description of the test beams at \mbox{DESY-II} can be found in reference~\cite{EUDET-2007-11}.


% In addition to measurements at DESY\,II, the beam telescopes were also characterised at other test beam facilities: 
% At CERN, the circular proton synchrotron PS~\cite{PS} of ?\,km length is a pre-accelerator for the SPS \cite{SPSP}, which in turn serves as an injector of proton beams for the Large Hadron Collider. 
% Additionally, it provides a proton beam on ? secondary targets resulting in a mixed beam (electrons, hadrons, muons) with energies between ??\,GeV and ??\,GeV
%  feeding up to ten ?? beam lines in the PS experimental area, one of them being the T9 ?? beam line. 
% One beam spill contains up to $\sim $?\,particles and is ?\,s to ?\,s long. 
% A spill occurs every ?\,s to ?\,s depending on the operation mode. 

%At SLAC, the Linac Coherent Light Source incorporates a primary electron beam with up to 13.6\,GeV and a repetition rate of 120\,Hz~\cite{SLAC}.
%Either this primary beam, or a secondary beam produced on a thin target can be sent to the End Station Test Beam (ESTB) with energies between 3.5\,GeV and 13.6\,GeV at 5\,Hz
% resulting in up to $10^{9}$ electrons per pulse.

%A beam pulse incorporates typically 109\,particles at 5\,Hz.\,\cite{d}
% https://portal.slac.stanford.edu/sites/ard_public/facet/newnav/Pages/tf/estb/ESTB-Beam.aspx

%Results on the resolution of the beam telescopes depending on different test beams and, thus, beam energies are described in section~\ref{sec:trackres}. 


==> content/results.tex <==


